CSEval: Towards Automated, Multi-Dimensional, and Reference-Free Counterspeech Evaluation using Auto-Calibrated LLMs

Counterspeech has emerged as a popular and effective strategy for combating online hate speech, sparking growing research interest in automating its generation using language models. However, the field still lacks standardised evaluation protocols and reliable automated evaluation metrics that align with human judgement. Current automatic evaluation methods, primarily based on similarity metrics, do not effectively capture the complex and independent attributes of counterspeech quality, such as contextual relevance, aggressiveness, or argumentative coherence. This has led to an increased dependency on labor-intensive human evaluations to assess automated counter-speech generation methods. To address these challenges, we introduce CSEval, a novel dataset and framework for evaluating counterspeech quality across four dimensions: contextual-relevance, aggressiveness, argument-coherence, and suitableness. Furthermore, we propose Auto-Calibrated COT for Counterspeech Evaluation (Auto-CSEval), a prompt-based method with auto-calibrated chain-of-thoughts (CoT) for scoring counterspeech using large language models. Our experiments show that Auto-CSEval outperforms traditional metrics like ROUGE, METEOR, and BertScore in correlating with human judgement, indicating a significant improvement in automated counterspeech evaluation.

==> sections/statisical_test.tex <==
\begin{table*}[h]
    \centering
    \label{tab:statistical_results}
    \begin{tabular}{lcccccccc}
        \toprule
        \textbf{Model} & \multicolumn{2}{c}{\textbf{Relevance Score}} & \multicolumn{2}{c}{\textbf{Aggressiveness Score}} & \multicolumn{2}{c}{\textbf{Coherence Score}} & \multicolumn{2}{c}{\textbf{Suitableness Score}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        & Mean & Std & Mean & Std & Mean & Std & Mean & Std \\
        \midrule
        BLEU\_1 & -0.007 & 0.022 & -0.147 & 0.043 & 0.115 & 0.040 & 0.005 & 0.025 \\
        ROUGE\_l & 0.213 & 0.037 & -0.167 & 0.020 & 0.354 & 0.027 & 0.200 & 0.027 \\
        METEOR\_score & 0.178 & 0.032 & -0.207 & 0.020 & 0.355 & 0.025 & 0.169 & 0.023 \\
        BERT\_score & 0.227 & 0.027 & -0.077 & 0.027 & 0.342 & 0.020 & 0.249 & 0.014 \\
        Toxicity & -0.019 & 0.030 & 0.272 & 0.018 & -0.184 & 0.037 & -0.107 & 0.028 \\
        BART\_score & 0.272 & 0.024 & -0.198 & 0.023 & 0.394 & 0.024 & 0.249 & 0.021 \\
        GPT-4 (zeroshot) & 0.529 & 0.031 & 0.336 & 0.061 & 0.444 & 0.025 & 0.422 & 0.039 \\
        GPT-4 (GEval) & 0.629 & 0.012 & 0.392 & 0.030 & 0.578 & 0.031 & 0.522 & 0.014 \\
        GPT-4 (Auto-CSEval) & 0.687 & 0.010 & 0.461 & 0.035 & 0.597 & 0.032 & 0.566 & 0.014 \\
        \bottomrule
    \end{tabular}
    \caption{Spearman ($\rho$) correlation results for selected methods based on statistical testing.}
\end{table*}



\begin{table*}[t]
    \centering
    \label{tab:statistical_delta}
    \resizebox{\textwidth}{!}{ % Resize table to fit within text width
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Model} & \multicolumn{1}{c}{\textbf{Relevance Score}} & \multicolumn{1}{c}{\textbf{Aggressiveness Score}} & \multicolumn{1}{c}{\textbf{Coherence Score}} & \multicolumn{1}{c}{\textbf{Suitableness Score}} \\
        \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
        & Mean & Mean & Mean & Mean \\
        \midrule
        Auto-CSEval - Best Traditional Metric & 0.415 & 0.189 & 0.202 & 0.317 \\
        Auto-CSEval - Best Method & 0.058 & 0.069 & 0.019 & 0.044 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Delta values comparing Auto-CSEval against the best traditional metric and best method across evaluation aspects.}
\end{table*}


==> tables/instructions_table.tex <==
\begin{table*}[t]
  \centering
  \begin{tabular}
  {lp{3cm}p{10cm}} 
    \toprule
    Task-ID & Generation Type & Instruction \\
    \midrule
    I$_1$ & Offensiveness & Analyze the offensiveness of the statement: \{\texttt{HS}\} \\
    \noalign{\vskip 1.0ex} % Space after the dashed line
    I$_2$ & Target Group & Identify the group of people that the speaker is targeting or discriminating against in the offensive statement: \{\texttt{HS}\} \\
    \noalign{\vskip 1.0ex} % Space after the dashed line
    I$_3$ & Speaker Intent & Analyze the speaker's intention behind writing the offensive statement: \{\texttt{HS}\} \\
    \noalign{\vskip 1.0ex} % Space after the dashed line
    I$_4$ & Power Dynamics & Explain the underlying power dynamics between the speaker and the target group in the offensive statement: \{\texttt{HS}\} \\
    \noalign{\vskip 1.0ex} % Space after the dashed line
    I$_5$ & Implication & Explain the implied meaning underlying the offensive statement: \{\texttt{HS}\} \\
    \noalign{\vskip 1.0ex} % Space after the dashed line
    I$_6$ & Emotional Reaction & Describe how the target group might feel emotionally after reading or listening to the offensive statement: \{\texttt{HS}\} \\
    \noalign{\vskip 1.0ex} % Space after the dashed line
    I$_7$ & Cognitive Reaction & Describe how the target group might react cognitively after reading or listening to the offensive statement: \{\texttt{HS}\} \\
    \midrule
    \noalign{\vskip 0.5ex}
    I$_8$ & Intent-Specific Counterspeech & Analyze the different aspects such as offensiveness, target group, stereotype, power dynamics, implied meaning, emotional, and cognitive reactions before writing a \{\texttt{INT}\} counterspeech for the offensive statement: \{\texttt{HS}\} \\
    \bottomrule
  \end{tabular}
% \caption{Instructions used for different tasks. Instructions \{I1, I2,..., I7\} correspond to each of the respective hate speech explanation dimensions of the Auxiliary Explanation Generation (AEG) task described under Section \ref{sec:phase1}. I8 describes the instruction used to train task-specific LoRA weights for intent-conditioned counterspeech generation, as described under Section \ref{sec:phase2}. {\texttt{HS}\} denotes the hate speech instance and {\texttt{INT}\} denotes the desired intent (Postive / Denoucing / Informative / Questioning)}
\caption{Detailed Instructions for the tasks of explanation and counterspeech generation respectively. The instructions labeled \{I$_1$, I$_2$, ..., I$_7$\} correspond with each of the dimensions of hate speech explanations in the Auxiliary Explanation Generation (AEG) task, as outlined in Section \ref{sec:phase1}. Instruction I$_8$ is crafted for training task-specific LoRA adapter for generating intent-conditioned counterspeech, detailed in Section \ref{sec:phase2}. In these instructions, {\texttt{HS}} represents the instance of hate speech, and {\texttt{INT}} denotes the targeted intent of the counterspeech, which includes \texttt{Positive}, \texttt{Denouncing}, \texttt{Informative}, or 
\texttt{Questioning}.}

\label{tab:instructions_table} % Label for the table
\end{table*}

==> tables/system_level_table.tex <==
\begin{table}[t!]
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c}
\toprule
\multicolumn{1}{l|}{\textbf{Metrics}} & \multicolumn{5}{c}{\textbf{Aspect-level preferencel}} \\
\midrule
 & \textbf{Rel $\uparrow$} & \textbf{Agg $\uparrow$} & \textbf{Coh $\uparrow$} & \textbf{Sui $\uparrow$} & \textbf{AVG $\uparrow$} \\
\midrule
Bleu & ${1}$ & $1$ & $1$ & $1$ & ${1}$ \\
ROUGE & ${1}$ & $1$ & $1$ & $1$ & ${1}$ \\
BertScore & ${1}$ & $1$ & $1$ & $1$ & ${1}$ \\
LLama-3 (G-EVAL) & ${1}$ & $1$ & $1$ & $1$ & ${1}$ \\
Mistral (G-EVAL) & ${1}$ & $1$ & $1$ & $1$ & ${1}$ \\
GPT-4 (G-EVAL) & ${1}$ & $1$ & $1$ 
& $1$ & ${1}$ \\
LLama-3 (Auto-CSEval) & ${1}$ & $1$ & $1$ & $1$ & ${1}$ \\
Mistral (Auto-CSEval) & ${1}$ & $1$ & $1$ & $1$ & ${1}$ \\
GPT-4  (Auto-CSEval) & ${1}$ & $1$ & $1$ & $1$ & ${1}$ \\

\bottomrule
\end{tabular}%
}
\end{center}
\caption{System-level ranking performance of LLM-based evaluators across different aspects. The ranking score is computed as NDCG score}
\label{tab:system_level_performance_table}
\vspace{-5mm}
\end{table}

==> tables/table1.tex <==
\begin{table*}[!ht]
\begin{center}
\small % Set the font size to small for the table content
\begin{tabular}{l}
\toprule
\textbf{Hate Speech:} All quite before the headscarves show up!  \\
\noalign{\vskip 0.5ex} % Space after the dashed line
\textbf{Generated CounterSpeech:} This seems to be based on a misconception. In reality, headscarves, such as hijabs, are often \\ worn for religious
reasons, primarily in Islamic culture, symbolizing modesty and personal conviction. This practice is \\ respected and protected in many countries
as part of religious freedom. Globally, the wearing of headscarves is not associated \\ 
with any form of disturbance or negativity but is a reflection
of cultural diversity and personal choice. \\
\noalign{\vskip 0.5ex} % Space after the dashed line
\textbf{Reference Counterspeech:} The idea about headscarves disrupting quietude is based on certain biases. Let's look at Indonesia,\\ the world's 
largest Muslim-majority country, where headscarves are commonplace. Far from causing disturbance, they are \\ a symbol of cultural identity and 
coexist with Indonesia's renowned social harmony. These examples show that headscarves \\ are part of societal diversity and acceptance,
not a source of disruption. \\
\noalign{\vskip 0.5ex} % Space after the dashed line
\midrule
\midrule
\textbf{Similarity-based Evaluators} \\
ROUGE-1: 0.44 \hspace{1cm} ROUGE-2: 0.25 \hspace{1cm} ROUGE-L: 0.42 \hspace{1cm} BERTScore: 0.24 \\
\noalign{\vskip 1.0ex} % Space after the dashed line
\midrule
\textbf{Single-dimensional Evaluators (predicted by three different evaluators)} \\
Consistency: 0.87 \hspace{1cm} Relevance: 0.74 \\
\noalign{\vskip 1.0ex} % Space after the dashed line
\midrule
\textbf{Unified Evaluator (predicted by UNiEVAL \cite{zhong-etal-2022-UniEVAL})} \\
Coherence: 0.04 \hspace{1cm} Consistency: 0.41 \hspace{1cm} Fluency: 0.92 \hspace{1cm} Relevance: 0.28 \\
\noalign{\vskip 1.0ex} % Space after the dashed line
\midrule
\textbf{LLM-based Evaluator (predicted by Auto-CSEval (GPT4))} \\
Relevance: 0.75 \hspace{1cm} Aggressiveness: 0.1 \hspace{1cm} Coherence: 0.8 \hspace{1cm} Suitability: 0.8 \\
\noalign{\vskip 1.0ex} % Space after the dashed line
\midrule
\textbf{Human Evaluation (Annotated by Experts, we map the scoring range to 0-1)} \\
Relevance: 0.8 \hspace{1cm} Aggressiveness: 0.25 \hspace{1cm} Coherence: 1.0 \hspace{1cm} Suitability: 1.0 \\ 
\bottomrule
\end{tabular}
\end{center}
\caption{An example of evaluating the counterspeech generation task. All metrics except BARTScore are scored in the range of 0 to 1, with higher scores indicating better quality. Our proposed Auto-CSEval is consistent with human evaluation, across multiple dimensions: Context Relevance, Aggressiveness, Argument Coherence, and Suitableness to evaluate the generated counterspeech. The scores predicted by Auto-CSEval are closer to human judgements.}
\label{tab:illustration_table}
\end{table*}
